Just-Right Consistency: reconciling availability and safety

By the CAP Theorem, a distributed data storage system can ensure either Consistency under Partition (CP) or Availability under Partition (AP), but not both. This has led to a split between CP databases, in which updates are synchronous, and AP databases, where they are asynchronous. However, there is no inherent reason to treat all updates identically: simply, the system should be as available as possible, and synchronised just enough for the application to be correct. We offer a principled Just-Right Consistency approach to designing such applications, reconciling correctness with availability and performance, based on the following insights:(i) The Conflict-Free Replicated Data Type (CRDTs) data model supports asynchronous updates in an intuitive and principled way.(ii) Invariants involving joint or mutually-ordered updates are compatible with AP and can be guaranteed by Transactional Causal Consistency, the strongest consistency model that does not compromise availability. Regarding the remaining, "CAP-sensitive" invariants:(iii) For the common pattern of Bounded Counters, we provide encapsulated data type that is proven correct and is efficient; (iv) in the general case, static analysis can identify when synchronisation is not necessary for correctness.Our Antidote cloud database system supports CRDTs, Transactional Causal Consistency and the Bounded Counter data type. Support tools help design applications by static analysis and proof of CAP-sensitive invariants. This system supports industrial-grade applications and has been tested experimentally with hundreds of servers across several geo-distributed data centres.

==> Makefile <==
# Important commands:
#	make update	# download repository version and merge
#	make commit	# upload to repository
#	make		# generate pdf
#	make bib	# generate bibliogrphy
#	make force	# generate bibliogrphy and force re-run
#	make clean	# remove temp files
#	make spotless   # idem + remove pdf, bib files

# Please do not add .pdf or other generated files to SVN targets.  Thanks!

FILE=RR-9145

MAKEFLAGS=	--no-print-directory

# ------------------------------
# User configurable dependencies
# ------------------------------

# GNUPlot source files
GPSOURCE= 
#	$(wildcard figures/*.gp)

# EPS files included
EPSSOURCE= 
#	$(wildcard figures/*.eps)

# PDF files included
PDFSOURCE= \
	couverture.pdf

# PNG files included
PNG= \
	logo-inria.png \
	pagei.png \
	rrpage1.png

# BIB files included
BIBS= \
	predef.bib \
	shapiro-bib-ext.bib \
	shapiro-bib-perso.bib \
	local.bib \
	Y1-dissemination.bib \
	Y2-dissemination.bib \
	Y3-dissemination.bib

# Bibtex style
BST= \
	abbrvnat-no-url.bst

# .tex file includes or inputs
TEXIN= RR.dtx RR.ins RR.sty

	# sig-alternate-05-2015.cls \
	# acmcopyright.sty

#	maths.sty \
	# $(wildcard *.cls) \
	# $(wildcard *.sty) \
	# $(wildcard tikzfigures/*.tex)

# other file dependencies
DEPS= Makefile

# files that are not Make dependencies but are required nonetheless
OTHERCOMMITS= \
	main.tex

	# books_app.tex \
	# ali-keep-safe.tex \
	# long-version-with-CRDTs+Antidote.tex \
	# word-count.numbers \

MANUALTARGET= \
	${PNG}

MANUALSOURCE= 


#
# MANUAL! add the following after default:
#
# figures/fig.png: figures/figures.key
# 	@echo "Must first recreate $@ from $<!!" 2>&1
# 	@false

# ------------------------------
# End user configurable dependencies
# ------------------------------

EPSGEN=$(GPSOURCE:.gp=.eps)
EPSGRAPHICS= ${EPSGEN} ${EPSSOURCE}

PDFGEN=$(EPSGRAPHICS:.eps=.pdf)
PDFGRAPHICS=${PDFGEN} ${PDFSOURCE}

GRAPHICSSOURCE= ${GPSOURCE} ${EPSSOURCE} ${PDFSOURCE} ${PNG}
GRAPHICSGEN=${EPSGEN} ${PDFGEN}

TEXTDEPS=${FILE}.tex ${TEXIN} ${DEPS} ${SNIPPETS}
GRAPHICDEPS= ${PDFGRAPHICS} ${PNG}

SOURCES= ${EPSSOURCE}  ${GPSOURCE}  ${EPSSOURCE}  ${PDFSOURCE}  ${PNG}  ${BIBS}  ${TEXIN} ${BST}
ALLFILES= ${FILE}.tex ${SOURCES} ${DEPS} ${MANUALSOURCE} ${MANUALTARGET} ${OTHERCOMMITS}

GNUPLOT= gnuplot 

# ------------------------------
# source control
# ------------------------------
default: etags pdf

snippets: ${SNIPPETS}

# MANUAL! uncomment:
${MANUALTARGET}: ${MANUALSOURCE}
	@echo "Must first recreate $@ from $<!!" 2>&1
	@false

pull update:
	svn update
#	git pull

push commit: ${MANUALTARGET}
	-svn propset svn:keywords 'URL Date Revision Author' ${FILE}.tex
# unset LANG because it influences the way SVN generates the date inside the file
# explicit ${ALLFILES} to verify that they have all been declared by 'svn add'
	unset LANG; svn commit -m '' ${ALLFILES}
	# git add ${ALLFILES}
	# git commit --allow-empty --allow-empty-message -m ""
	# git push origin master
# also commit files not in dependencies
	unset LANG; svn commit -m ''
	# git add -u
	# git commit --allow-empty --allow-empty-message -m ""
	# git push origin master

spotless:: clean

# begin diff
# requires latexdiff from http://www.ctan.org/tex-archive/support/latexdiff/
diff: diff-$(FILE)-diff.pdf

# remotebase svnbase:
# 	svn cat $(FILE).tex > $(FILE)-base.tex

# localbase base savebase:
# 	cp $(FILE).tex $(FILE)-base.tex

diff-$(FILE)-diff.tex: ${V1}.tex $(FILE).tex
	latexdiff ${V1}.tex $(FILE).tex > diff-$(FILE)-diff.tex

diff-$(FILE)-diff.aux: $(FILE).aux
	cp $(FILE).aux diff-$(FILE)-diff.aux

diff-$(FILE)-diff.bbl: $(FILE).bbl
	cp $(FILE).bbl diff-$(FILE)-diff.bbl

diff-$(FILE)-diff.pdf: diff-$(FILE)-diff.tex diff-$(FILE)-diff.aux diff-$(FILE)-diff.bbl
	pdflatex diff-$(FILE)-diff.tex
	pdflatex diff-$(FILE)-diff.tex

clean::
	-rm -f diff-$(FILE)-diff.* 

# end diff

# ---------- latex compilation ----------

tags etags: TAGS

TAGS: ${TEXTDEPS} 
	etags ${TEXTDEPS}

clean::
	rm -f TAGS

graphics: epsgraphics pdfgraphics

epsgraphics: ${EPSGRAPHICS}

pdfgraphics: ${PDFGRAPHICS}

# dvi: $(FILE).dvi 

edit:
	open ${FILE}.tex

show: pdf
	open $(FILE).pdf

pdf: $(FILE).pdf

print lpr: $(FILE).pdf
	lpr $(FILE).pdf

# $(FILE).dvi: $(FILE).tex $(FIGS)

aux: $(FILE).aux

$(FILE).pdf ${FILE}.aux: ${TEXTDEPS} ${GRAPHICDEPS}
	pdflatex $(FILE)

### $(FILE).dvi ${FILE}.aux: ${FILE}.tex ${DEPS} ${EPSGRAPHICS} ${PNG}
### 	latex $(FILE)

#figs:
#		( cd figs; $(MAKE) )
clean::
		/bin/rm -f *~ *.bak *.aux *.log *.toc *.lof *.dvi *.bbl *.blg *.lot *.out
		/bin/rm -rf auto/

spotless:: 
		/bin/rm -f ${FILE}.pdf

# ---------- bibliography ----------

force: bib forcepdf1 default forcepdf2

forcepdf1 forcepdf2: FORCE
	pdflatex $(FILE)

FORCE:

${FILE}.bbl: aux ${BST} ${BIBS} 
		-bibtex ${FILE}
#		./bibnourl.sh ${BIBS}
#		BIBINPUTS=tmp/:$$BIBINPUTS bibtex $(FILE)
#		sed -e 's/%//g' < $(FILE).bbl > $(FILE).bbl~
#		mv $(FILE).bbl~ $(FILE).bbl

# clean::
# 	rm -rf tmp/

bib: $(FILE).bbl 

# effective only for user @shapiro
ifeq ($(shell whoami),shapiro)
shapiro-bib-ext.bib: /Users/shapiro/svnbackup/bib/shapiro-bib-ext.bib
	cp -p /Users/shapiro/svnbackup/bib/shapiro-bib-ext.bib .

shapiro-bib-perso.bib: /Users/shapiro/svnbackup/bib/shapiro-bib-perso.bib
	cp -p /Users/shapiro/svnbackup/bib/shapiro-bib-perso.bib .

predef.bib: /Users/shapiro/svnbackup/bib/predef.bib
	cp -p /Users/shapiro/svnbackup/bib/predef.bib .

short-predef.bib: /Users/shapiro/svnbackup/bib/short-predef.bib
	cp -p /Users/shapiro/svnbackup/bib/short-predef.bib .

grassroots.bib: /nobackup/svnstuff/syncfree_SVN/papers/grassroots.bib
	ln -s /nobackup/svnstuff/syncfree_SVN/papers/grassroots.bib .

spotless::
	rm -f shapiro-bib-perso.bib shapiro-bib-ext.bib predef.bib short-predef.bib grassroots.bib
endif
# end only @shapiro

# ---------- html ----------

html: ${FILE}.html

${FILE}.html ${FILE}.css: ${FILE}/${FILE}.html
	cp -p ${FILE}/${FILE}.html .
	cp -p ${FILE}/${FILE}.css .

${FILE}/${FILE}.html: ${FILE}.aux
	latex2html -split 0 ${FILE}

clean::
	rm -rf ${FILE}/

spotless::
	rm -f ${FILE}.html ${FILE}.css

# ---------- standard targets ----------

%.eps: %.obj
	tgif -print -eps $^
%.eps: %.gp
	$(GNUPLOT) $^

# %.eps: %.gp dat/%.dat
#	$(GNUPLOT) $^

%.eps: %.fig
	fig2dev -L eps $^ >$@
%.eps: %.prn
	ps2epsi $^ $@
clean::
	rm -f ${GRAPHICSGEN}

%.eps: %.dia
	dia -e $@ $^
%.eps: %.epsraw
	ps2epsi $^ $@

%.pdf: %.tex
	pdflatex $^

%.bbl: %.aux
	-bibtex $^

# According to ACM instructions, '-P cmz' embeds Type 1 fonts, which
# enables later PDF generation to be of higher quality 
# %.ps: %.dvi
# 	dvips -P cmz $^ -o
# 	rm -f $@.gz

%.pdf: %.ps
	ps2pdf $^
%.pdf: %.eps
	epstopdf $^

tgz: ${FILE}.pdf
	dir=`basename $$PWD`; \
	tar czvf /tmp/$(FILE).tgz -C .. \
	$(patsubst %,$$dir/%,\
	    ${FILE}.pdf \
	    ${ALLFILES} \
	    ${patsubst %,dat/%,${GPSOURCE:.gp=.dat}}\
	)

zip: ${FILE}.pdf
	rm -rf /tmp/$(FILE).zip; \
	zip /tmp/$(FILE).zip \
	    ${FILE}.pdf \
	    ${ALLFILES} \
	    ${patsubst %,dat/%,${GPSOURCE:.gp=.dat}}



